Analyzing the Robustness of Nearest Neighbors to Adversarial Examples

Motivated by safety-critical applications, test-time attacks on classifiers via adversarial examples has recently received a great deal of attention. However, there is a general lack of understanding on why adversarial examples arise; whether they originate due to inherent properties of data or due to lack of training samples remains ill-understood. In this work, we introduce a theoretical framework analogous to bias-variance theory for understanding these effects. We use our framework to analyze the robustness of a canonical non-parametric classifier - the k-nearest neighbors. Our analysis shows that its robustness properties depend critically on the value of k - the classifier may be inherently non-robust for small k, but its robustness approaches that of the Bayes Optimal classifier for fast-growing k. We propose a novel modified 1-nearest neighbor classifier, and guarantee its robustness in the large sample limit. Our experiments suggest that this classifier may have good robustness properties even for reasonable data set sizes.

==> summary.tex <==
\section{Summary of Results}
\label{sec:summary}

This section gives a summary of the main results and also provides a
table (see Figure~\ref{fig:table-notation}) of all the important
notation used throughout the paper.

%% Table of notation

\begin{figure*}
\begin{center}
\begin{tabular}{|c|l|} \hline \hline
{\sf Notation} & {\sf Description} \\ \hline \hline
$\calX$ & Instance space \\ \hline
$\calY$ & Label space \\ \hline
$D$ & Distribution over $\calX \times \calY$ \\ \hline
$\mu$ & the marginal of $D$ over $\calX$ \\ \hline
$\eta$ & the conditional distribution of the labels \\
  & given an instance $x$ \\ \hline
$g$ & the Bayes optimal classifier \\ \hline
Robustness radius $\rho(f, x)$ & 
$\inf_{r > 0} \{ \exists x' \in \calX \cap B(x, r) {\text{\ s.t\ }} f(x) \neq f(x') \}$ \\ \hline
Robustness $R(f, r, \mu)$ with respect to a  &
$\Pr_{x \sim \mu} ( \{ x | \rho(f, x) \geq r \} )$  \\ 
distribution $\mu$ & \\ \hline
  
R-accuracy $\racc_{D}$ of a classifier $f$ & $\Pr_{x \sim \mu}(\{ x | f(x) = g(x), \rho(f, x) \geq r \})$\\
\hline
$B(x, \Delta)$ & closed ball around $x$ of radius $\Delta$ \\ \hline
$B^o(x, \Delta)$ & open ball around $x$ of radius $\Delta$ \\ \hline
\end{tabular}
\end{center}
\caption{Some important notation used throughout the paper.}
\label{fig:table-notation}
\end{figure*}


%% Main results of section 3
\vspace{5pt}
\noindent {\bf Analysis.}  Section~\ref{sec:nnanalysis} presents a
robustness analysis of the nearest-neighbor (NN) binary classifier
(i.e. the labels are $0$ or $1$). The first result in this section
shows that if 1) the density of $x$ and the conditional distribution of $y$ given $x$ are continuous and 2) $\eta(x) = \Pr(y
= 1 | x) \in (0, 1)$, then the radius of robustness of the
NN-classifier at $x$ tends to $0$ as $n \rightarrow \infty$ (where $n$
is the number of points). We also demonstrate that a similar result
also holds for $k$-nearest neighbors ($k$-NN) for a fixed $k$.  This means NN is inherently non-robust in the region where $\eta(x)\in(0,1)$, whereas accuracy still holds. Next we
consider the case when NN is actually robust, and show that this
happens in the {\em{interior}} of a region where $\eta(x) = 0$ or
$1$. Detailed exposition of these results are provided in the section.

%% Main results from section 4
\vspace{5pt}
\noindent
{\bf Algorithm.}
Motivated by the discussion in Section~\ref{sec:nnanalysis},
Section~\ref{sec:robustnn} presents our new algorithm that achieves
robustness and classification accuracy. Here we only provide an
intuition behind our algorithm and details can be found in the
section. Assume we are given a set $\labeledsample$. A subset
$S \subseteq \labeledsample$ is called $r$-separated if for 
all points $(x,y)$ and $(x',y')$ in $S$, $d(x,x') \leq r$ implies that
label of $y = y'$ (in other words, points that are ``close'' have the 
same label). The cover induced by $S$ is the union of closed balls for
all elements in $S$ and is given by the following 
equation:
\begin{eqnarray*}
Cover(S, \Delta) & = & \bigcup_{x \in S} B(x, \Delta)
\end{eqnarray*}
Note that the probability measure of $Cover(S, \Delta)$ can be
computed as $\sum_{s \in S} D( B(x, \Delta))$ if $S$ is $z$-separated
(if $z > 2 \Delta$ then essentially all the balls are
disjoint). Roughly speaking, our problem can be stated as follows:
\begin{quote}
Given a robustness radius $r$ and tolerance parameter $\Delta$, find a
$2r+2\Delta$-separated subset $S$ of $\labeledsample$ that maximizes
the probability measure of $Cover(S, \Delta)$.
\end{quote}
A 1-NN classifier trained on such an $S$ will be highly robust. 
Notice that even if the distribution $D$ is given (in general the distribution $D$ is unknown), the problem is $NP$-hard. Our algorithm can be viewed as
an approximation algorithm for this problem.

%% Main results of the section 5

%% Main results of the experiments Section 6
\vspace{5pt}
\noindent {\bf Evaluation.}  We validate the effectiveness of our
defense mechanism against both white-box and black-box attacks on
three different datasets.  Our defense mechanism achieves the highest
classification accuracy in all adversarial settings when the training
sample is dense in the input space, a scenario in which the
nearest-neighbor classifier is most effective. It also provides more
robustness on relatively sparse training set when the perturbation
magnitude is large enough to pose a serious threat. Details of our 
evaluation are presented in Section~\ref{sec:exp}.
%(Other benefits of our mechanism is: attack-agnostic, faster
%in the inference/prediction stage compared to adversarial training.)


